Robust guarantees for learning an autoregressive filter

The optimal predictor for a linear dynamical system (with hidden state and Gaussian noise) takes the form of an autoregressive linear filter, namely the Kalman filter. However, a fundamental problem in reinforcement learning and control theory is to make optimal predictions in an unknown dynamical system. To this end, we take the approach of directly learning an autoregressive filter for time-series prediction under unknown dynamics. Our analysis differs from previous statistical analyses in that we regress not only on the inputs to the dynamical system, but also the outputs, which is essential to dealing with process noise. The main challenge is to estimate the filter under worst case input (in $\mathcal H_\infty$ norm), for which we use an $L^\infty$-based objective rather than ordinary least-squares. For learning an autoregressive model, our algorithm has optimal sample complexity in terms of the rollout length, which does not seem to be attained by naive least-squares.

==> discussion.tex <==
\section{Discussion and future work}

Note that in order to have concentration, we require $\wt \Om(r)$ rollouts of each frequency. Ideally, we would be able to obtain bounds even with fewer rollouts, or with just 1 rollout for a long period of time.  Small-ball inequalities can be used as in \cite{simchowitz2018learning} to show that $g^{(j)}_{LS},h^{(j)}_{LS}$ does well on the frequencies $\fc{2\pi j}{cr}$. However, they do not provide the uniform bounds needed to show that $(g,h)$ defined as in~\eqref{e:ls} also do well. We leave this line of investigation to future work.


==> lb.tex <==
\section{Lower bound}

We show that the factor of $\ve{H^*}_\iy \ve{H_{\textrm{unr}}^*}_\iy$ is unavoidable in Theorem~\ref{t:main-trunc}.



==> proof.tex <==
\section{Proof}
\label{s:proof}


%%%%%%%%%%%%
\begin{comment}
It will be convenient to first prove the theorem in the case when the burn-in time is infinite. Note that by the stability assumption on $H^*_{\textrm{unr}}$, for signals $\ve{x}_\iy$, the outputs will not diverge.
\begin{thm}\label{t:main}
Theorem~\ref{t:main-trunc} holds in the setting when the burn-in time $L$ is infinite.
%There is $C,C'$ such that the following holds.
%Consider the system~\eqref{e:ar-sys}. 
%Suppose that $\ve{H}_{\iy}<1$. 
%%Suppose that $\ve{\hunr}_1\le L$. 
%Algorithm~\ref{a:ls} with $c\ge 8\pi$,  rollout length $T$, and $\ell \ge \max\{T/c,C^{\prime2}(r+\ln \prc{\de})\}$ rollouts  of each input, with probability $1-\de$, returns $g,h$ such that 
%\begin{align}
%\ve{(G-G^*) + (H-H^*)H^*_{\textrm{unr}}G^*}_\iy &\le 
%\fc{C}{\sqrt{\ell T}}\pa{\ln \pf{\ell rT}{\de}}^{\fc 32}(1+\ve{H^*}_\iy)\ve{H^*_{\textrm{unr}}}_\iy=:\ep_1
%\\
%\ve{(H-H^*)H^*_{\textrm{unr}}}_2 &\le 
%\fc{C}{\sqrt{c\ell T}}\pa{\ln \pf{\ell rT}{\de}}^{\fc 32}=:\ep_2.
%%\ve{(g-g^*,h-h^*)}_{\cL,\cH_\iy} &\le O\pf{\ln \pf{cTr}{\de}\ve{H_{\textrm{unr}}}_{\iy}}{\sqrt{\ell r}}.
%\end{align}
%Therefore, with probability $1-\de$, 
%\begin{align}
%\E\ba{\sumo tT \ve{y_{\text{err}}(t)}^2} 
%&\le \ep_1^2 \ve{x}_2^2 + \ep_2^2T.
%\end{align}
\end{thm}
\end{comment}

%We prove Theorem~\ref{t:main-trunc}. We break the proof into 4 parts. The first 3 parts will prove Theorem~\ref{t:main}.
Our proof for Theorem~\ref{t:main} consists of 3 parts.
\begin{enumerate}
\item
\ul{Concentration:} 
If $\ol y=M^\top x$ and $y=\ol y+\eta$, then the error from least-squares $\amin_x\ve{M^\top x-y}^2$ is $(MM^\top)^{-1}M\eta$. A simple way to bound this is to bound $MM^{\top}$ from below and $M\eta$ from above. When we have $s$ samples, and $x\in \R^r$, we expect $\ve{(MM^\top)^{-1}} \le O(\prc{s})$ and $\ve{M\eta}\le O\pa{\sqrt{rs}}$.

We show that the matrices $Q^{(\bullet)}:=\sumo k{c\ell r}
 M^{(\bullet,k)} M^{(\bullet,k)\top}$ and $Q^{(j)}:=\sumo k{\ell} (M^{(j,k)}_{\cos}M^{(j,k)\top}_{\cos} + M^{(j,k)}_{\sin}M^{(j,k)\top}_{\sin})$
in the least-squares problem concentrate using matrix concentration bounds (Lemma~\ref{l:mat-conc}), and that the terms such as $\sumo k{c\ell r} M^{(\bullet,k)}\eta^{(\bullet, k)}$
%$\sumo k{\ell}\sumo t{T} [M^{(j,k)}_{\cos,t} \eta^{(j,k)}_{\cos}(t) + M^{(j,k)}_{\cos,t} \eta^{(j,k)}_{\sin}(t)]$ 
concentrate by martingale concentration (Lemma~\ref{l:vec-conc}). The main complication is to track how the error $h_{LS}-h^*$ propagates into $g^{(j)}_{LS}-g^*$ (see~\eqref{e:proj-g-h} and following computations).
\item
\ul{Generalization:} The bounds we obtain on $\coltwo{g^{(j)}_{LS}}{h_{LS}} - \coltwo{g^*}{h^*}$ in the direction of the $j$th frequency~\eqref{e:jgh} show that the actual solution $(g^*,h^*)$ does well in the min-max problem~\eqref{e:ls}. The solution $(g,h)$ to~\eqref{e:ls} will only do better. By concentration, the matrices in the least-squares problem $Q^{(\bullet)}$, $Q^{(j)}$ and in the actual expected square loss are comparable. Because $(g,h)$ does well in the min-max problem, it will do comparably well with respect to the actual expected loss, when the input is one of the frequencies that has been tested, $\fc{2\pi j}{cr}$. 

In this step, we already have enough to bound $\ep_2$, the error in estimation with pure noise and no input signal.
\item
\ul{Interpolation:} We've produced $(g,h)$ that is close to the actual $(g^*,h^*)$ when tested on each of the frequencies $\fc{2\pi k}{cr}$, but need to extend it to all frequencies. Considering transfer functions and clearing denominators, this reduces to a problem about polynomial interpolation. We use a theorem from approximation theory (Theorem~\ref{l:interp}) that bounds the maximum of a polynomial $p$ on the unit circle, given its value at $\ge \deg p$ equispaced points. Note that it is crucial here that the number of parameters in $g,h$ is less than the number of frequencies tested. 

Note that we needed to clear $1-z^{-1}H^*$ from the denominator, so we lose a factor of $\ve{H_{\textrm{unr}}^*}_{\iy} = \ve{1-z^{-1}H^*}_{\iy}$ here. We get a bound on $\ep_1$, finishing the proof of Theorem~\ref{t:main}.
%\item
%\ul{Truncation:} Finally, we show that with a large burn-in time, the distribution of $y$'s will be almost indistinguishable from the steady-state distribution, and hence the algorithm still works.
\end{enumerate}

\subsection{Concentration}

%\fixme{Mention something about small-ball---why we can't use it naively here.}
We first set up notation and make some preliminary observations.
Let $\mathbf X^{(j)}_{\cos}\in \R^{r\times T}$ be the matrix with columns $x^{(j,k)}_{\cos}(t-1:t-r)$, $1\le t\le T$ and likewise define $\mathbf X^{(j)}_{\sin}, \mathbf Y^{(j,k)}_{\cos}, \mathbf Y^{(j,k)}_{\sin}$, so that 
$M^{(j,k)}_* = \coltwo{\mathbf X^{(j)}_*}{\mathbf Y^{(j)}_*}$ for $*\in \{\cos,\sin\}$.
Let 
$\Ga^{(\bullet)} = \E_{\eta^{(\bullet,k)}} M^{(\bullet, k)}M^{(\bullet, k)\top}$, $\Ga^{(j)}_{*,t}=\E_{\eta^{(j,k)}}M^{(j,k)}_{*,t} M^{(j,k)\top}_{*,t}$, $\Ga^{(j)}_{X,*,t}=\mathbf X^{(j)}_{*,t}\mathbf X^{(j)\top}_{*,t}$ where $*\in \{\cos,\sin\}$, $\eta^{(\bullet,k)},\eta^{(j,k)}_{*}$ is the noise in the various rollouts. 

%the covariance of $M^{(\bullet,k)}$, $M^{(j,k)}_{\cos, t}$, $M^{(j,k)}_{\sin ,t}$, $\mathbf X^{(j,k)}_{\cos, t}$, $\mathbf X^{(j,k)}_{\sin,t}$ be $\Ga^{(\bullet)}$, $\Ga^{(j)}_{\cos, t}$, $\Ga^{(j)}_{\sin, t}$, $\Ga^{(j)}_{X,\cos,t}$, $\Ga^{(j)}_{X,\sin, t}$ respectively. Note that this is periodic with period dividing $cr$. 
Let $\Ga^{(j)} = %\rc{cr}\sumo t{cr}
\Ga^{(j)}_{\cos, t} + \Ga^{(j)}_{\sin, t}$ and $\Ga^{(j)}_X=\Ga^{(j)}_{X,\cos, t} + \Ga^{(j)}_{X,\sin,t}$.
They do not depend on $t$, which can be seen as follows. Consider the system response to $x^{(j)}(t)=e^{2\pi i jt}{cr}$. (Although we cannot put in complex values in the system, there is a well-defined response for complex inputs.) Let $M^{(j)}$ be the matrix with columns $M^{(j)}_t=\coltwo{x^{(j)}(t-1:t-r)}{y^{(j)}(t-1:t-r)}$, where the $y^{(j)}$ is defined as in~\eqref{e:ar-sys} except with noise equal to $\eta^{(j)}(t)=\eta^{(j)}_{\cos}(t)+i\eta^{(j)}_{\sin}(t)$, $\eta^{(j)}_{\cos}(t), \eta^{(j)}_{\sin}(t)\sim N(0,1)$. Because $M^{(j)}_{t+s}$ has the same distribution as $e^{\fc{2\pi i s}{cr}}M^{(j)}_t$, the expression $\E [M^{(j)}_tM^{(j)\dagger} + M^{(-j)}_tM^{(-j)\dagger}_t]$ does not depend on $t$. Expanding, it equals $\rc 2\E[(M^{(j)}_{\cos, t}+iM^{(j)}_{\sin, t})(M^{(j)}_{\cos, t}-iM^{(j)}_{\sin, t})^\top + 
(M^{(j)}_{\cos, t}-iM^{(j)}_{\sin, t})(M^{(j)}_{\cos, t}+iM^{(j)}_{\sin, t})^\top] = \Ga^{(j)}_{\cos,t}+\Ga^{(j)}_{\sin,t}$. Similarly, $\Ga^{(j)}_X$ is well-defined. Note that $\Ga_X$ has rank $\le 2$, as it is spanned by $x^{(\pm j)}(r:1)$. 

%; by calculation they do not depend on $t$. %it is the same for any $t$. 
%\fixme{Explain?}
%$\mathbf Y^{(j,k)}_{\cos}$ be the matrix with columns $
Let \begin{align}
Q^{(\bullet)} &=
 \sumo k{c\ell r}
 M^{(\bullet,k)} M^{(\bullet,k)\top}
=
 \sumo k{c\ell r}  \sumo tT M^{(\bullet,k)}_t M^{(\bullet,k)\top}_t
 \\
%Q^{(j)}_X &= 
%%\sumo k{cr} 
%\ell \pa{\mathbf X^{(j,k)}_{\cos}\mathbf X^{(j,k)\top}_{\cos} + 
%\mathbf X^{(j,k)}_{\sin}\mathbf X^{(j,k)\top}_{\sin}}
%\\
Q^{(j)} &= 
\sumo k{\ell} (M^{(j,k)}_{\cos}M^{(j,k)\top}_{\cos} + M^{(j,k)}_{\sin}M^{(j,k)\top}_{\sin}) =
\sumo k\ell \sumo tT (M^{(j,k)}_{\cos,t}M^{(j,k)\top}_{\cos,t} + M^{(j,k)}_{\sin,t}M^{(j,k)\top}_{\sin,t}).
\end{align}
We calculate the least squares solution $h_{LS}$ and the error $h_{LS}-h^*$:
\begin{align}
h_{LS} &= Q^{(\bullet)-1}\sumo k{c\ell r} M^{(\bullet,k)} y^{(\bullet,k)}\\
h^*&= Q^{(\bullet)-1} \sumo k{c\ell r} M^{(\bullet,k)} \ol y^{(\bullet,k)}\\
h_{LS}-h^*&=Q^{(\bullet)-1} \sumo k{c\ell r} M^{(\bullet,k)} \eta^{(\bullet,k)}\\
&=\Ga^{(\bullet)-\rc 2}
\ub{(\Ga^{(\bullet)-\rc 2}Q^{(\bullet)} \Ga^{(\bullet)-\rc 2})^{-1}}{(0\bullet)}
\ub{\Ga^{(\bullet)-\rc 2}\sumo k{c\ell r} M^{(\bullet, k)}\eta^{(\bullet,k)}}{(1\bullet)}
\label{e:h-err}
\end{align}
The least squares solution $g^{(j)}_{LS}$ is
\begin{align}
g^{(j)}_{LS} &=
\rc{\ell T} \Ga^{(j)+}_X
\ba{
\sumo k{\ell} 
[\mathbf X^{(j)}_{\cos}(y^{(j,k)}_{\cos} - \mathbf Y^{(j,k)}_{\cos}h_{LS})+
\mathbf X^{(j)}_{\sin}(y^{(j,k)}_{\sin} - \mathbf Y^{(j,k)}_{\sin}h_{LS})]
}.\label{e:ls-g}
\end{align}
We calculate
\begin{align}
y^{(j,k)}_{\cos} - \mathbf Y^{(j,k)}_{\cos}h_{LS}&=
\eta^{(j,k)}_{\cos} + \ol y_{\cos}^{(j,k)} - \mathbf Y^{(j,k)\top}_{\cos}h^* - \mathbf Y^{(j,k)\top}_{\cos}(h_{LS}-h^*)\\
&=
\eta^{(j,k)}_{\cos} + \mathbf X^{(j)\top}_{\cos} g^* - \mathbf Y^{(j,k)\top}_{\cos}(h_{LS}-h^*)
\label{e:h-diff-calc}
\end{align}
and the analogous equations for $\sin$. Substituting~\eqref{e:h-diff-calc} into~\eqref{e:ls-g}, letting $P^{(j)}_X$ be the projection onto the column space of $\Ga^{(j)}_X$,  and noting $\rc{\ell T}\Ga^{(j)+}\sumo k{\ell}(\mathbf X^{(j)}_{\cos}\mathbf X^{(j)}_{\cos} + \mathbf X^{(j)}_{\sin}\mathbf X^{(j)}_{\sin})g^*=P^{(j)}_Xg^*$, we get
\begin{align}
g^{(j)}_{LS} &= P^{(j)}_X g^* + 
\rc{\ell T} \Ga^{(j)+}_X 
\ba{
\sumo k{cr}[ \mathbf X^{(j)}_{\cos} (\eta^{(j,k)}_{\cos} + \mathbf Y^{(j,k)\top}_{\cos}(h_{LS}-h^*)) + \mathbf X^{(j)}_{\sin} (\eta^{(j,k)}_{\sin} + \mathbf Y^{(j,k)\top}_{\sin}(h_{LS}-h^*))]
}
\end{align}
Then the error in $\coltwo{g^{(j)}_{LS}}{h_{LS}}$ together (projected with $P^{(j)}_X$) is
\begin{align}
\label{e:proj-g-h}
&
\matt{P^{(j)}_X}OO{I_r}
\ba{
\coltwo{g^{(j)}_{LS}}{h_{LS}} - \coltwo{g^*}{h^*}
}\\
\quad&=\coltwo{\rc{\ell T} \Ga^{(j)+}_X\sumo k{\ell}[ \mathbf X^{(j)}_{\cos} (\eta^{(j,k)}_{\cos} + \mathbf Y^{(j,k)\top}_{\cos}(h_{LS}-h^*)) + \mathbf X^{(j)}_{\sin} (\eta^{(j,k)}_{\sin} + \mathbf Y^{(j,k)\top}_{\sin}(h_{LS}-h^*))]}{h_{LS}-h^*}
\end{align}
We don't care about the absolute error of this, which can be large; we just care about the mean error on the inputs $x^{(j)}_{\cos}$ and $x^{(j)}_{\sin}$. Let $\mathbf Y^{(j)}_{\cos}$ be the matrix with the mean responses to $x^{(j)}_{\cos}$, $\mathbf Y^{(j)}_{\cos,t} = \ol y^{(j)}_{\cos}(t-1:t-r)$,
and likewise for $\sin$. Write $\mathbf Y^{(j,k)}_{\cos} = \mathbf Y^{(j)}_{\cos}  + \mathbf N^{(j,k)}_{\cos}$, etc., where $\mathbf  N^{(j,k)}_{\cos}$ is the noise term.
Then
\begin{align}
&
\pa{x^{(j)}_{\cos}(r:1)^{\top} \; \ol y^{(j)}_{\cos}(r:1)^\top}
%\pa{\mathbf X^{(j)\top}_{\cos}\; \mathbf Y^{(j)\top}_{\cos}}
\ba{\coltwo{g^{(j)}_{LS}}{h_{LS}}  - \coltwo{g^*}{h^*} }\\
&=
%\mathbf X^{(j)\top}_{\cos} 
x^{(j)}_{\cos}(r:1)^{\top}\rc{\ell T} \Ga^{(j)+}_X 
\ba{\sumo k{\ell} \mathbf X^{(j,k)}_{\cos}\eta^{(j,k)}_{\cos} +
 \mathbf X^{(j)}_{\sin}\eta^{(j,k)}_{\sin} }\\
 &\quad +
 \ba{x^{(j)}_{\cos}(r:1)^{\top} \rc{\ell T} \Ga^{(j)+}_X
  \ba{-\sumo k{\ell}( \mathbf X^{(j)}_{\cos}\mathbf Y^{(j,k)\top}_{\cos} +
 \mathbf X^{(j)}_{\sin}\mathbf Y^{(j,k)\top}_{\sin} )}
 +
 %\mathbf Y^{(j)\top}_{\cos}
\ol y^{(j)}_{\cos}(r:1)^\top}
 (h_{LS}-h^*)\\
 &=
%\mathbf X^{(j)\top}_{\cos} 
x^{(j)}_{\cos}(r:1)^{\top}
\rc{\ell T} \Ga^{(j)+}_X
\ba{\sumo k{\ell} \mathbf X^{(j,k)}_{\cos}\eta^{(j,k)}_{\cos} +
 \mathbf X^{(j)}_{\sin}\eta^{(j,k)}_{\sin} }\\
 &\quad +
 \ba{%\mathbf X^{(j)\top}_{\cos} 
 x^{(j)}_{\cos}(r:1)^{\top}
 \rc{\ell T} \Ga^{(j)+}_X
  \ba{-\sumo k{\ell}( \mathbf X^{(j)}_{\cos}\mathbf N^{(j,k)\top}_{\cos} +
 \mathbf X^{(j)}_{\sin}\mathbf N^{(j,k)\top}_{\sin} )}
}
 (h_{LS}-h^*)
\label{e:canc} \\
 &\quad \text{(see explanation below)}\nonumber\\
 &=\rc{\ell T} 
% \mathbf X^{(j)\top}_{\cos}
x^{(j)}_{\cos}(r:1)^{\top}
\Ga^{(j)+\rc 2}_X \Bigg[
\ub{ \Ga^{(j)+\rc 2}_X \sumo k\ell (\mathbf X^{(j)}_{\cos} \eta^{(j,k)}_{\cos} + \mathbf X^{(j)}_{\sin} \eta^{(j,k)}_{\sin})}{(1)} 
\label{e:gh-err}
\\
&\quad + 
\ub{ \Ga^{(j)+\rc 2}_X \sumo k\ell (\mathbf X^{(j)}_{\cos} \mathbf N^{(j,k)}_{\cos} + \mathbf X^{(j)}_{\sin} \mathbf N^{(j,k)}_{\sin})(h_{LS}-h^*)}{(2)}
 \Bigg]
 \label{e:gh-err2}
\end{align}
In~\eqref{e:canc} we used that $x^{(j)}_{\cos}(r:1)^\top  \Ga^{(j)+}_X\ba{-
\sumo k{\ell} \mathbf X^{(j)}_{\cos}
\mathbf Y^{(j)}_{\cos} + 
\mathbf X^{(j)}_{\sin}
\mathbf Y^{(j)}_{\sin} 
}+\ol y^{(j)}_{\cos}(r:1)^\top=0$. To see this, let $A$ be the matrix taking $x^{(j)}_{*}(t-1:t-r)\mapsto \ol y^{(j)}_{*}(t-1:t-r)$ for $*\in \{\cos,\sin\}$. Then this is $x^{(j)}_{\cos}(r:1)^\top \Ga^{(j)+}_X\ba{-\sumo k{\ell}\sumo tT (\mathbf X^{(j)}_{\cos,t}\mathbf X^{(j)\top}_{\cos,t}+\mathbf X^{(j)}_{\sin,t}\mathbf X^{(j)\top}_{\sin,t})A^\top}+x^{(j)}_{\cos}(r:1)^\top A^\top=0$.

In Section~\ref{s:mat-conc} we lower bound $(0\bullet)$ in~\eqref{e:h-err}, and
%$Q^{(j)+}$, and 
in Section~\ref{s:vec-conc} we upper bound % and
$(1\bullet), (1)$ in~\eqref{e:h-err} and~\eqref{e:gh-err}. In Section~\ref{s:tog} we bound (2) in~\eqref{e:gh-err} and put the bounds together to obtain (for some $C_7$),
\begin{align}
\ve{\Ga^{(j)\rc 2}\ba{\coltwo{g^{(j)}_{LS}}{h_{LS}}  - \coltwo{g^*}{h^*} }}
&\le \fc{C_7}{\sqrt{\ell T}}\pa{\ln \pf{\ell rT}{\de}}^{\fc 32}
\label{e:gagh0}
\end{align}
%$M^{(j,k)}_{\cos,t} \ol y^{(j,k)}_{\cos}(t)
%+ M^{(j,k)}_{\sin,t} \ol y^{(j,k)}_{\sin}(t)$.

%Let $P^{(j)}$ be the projection onto the column space of $Q^{(j)}$.
%Then the least-squares solutions are
%\begin{align}
%\coltwo{g^{(\bullet)}_{LS}}{h^{(\bullet)}_{LS}}
%&= Q^{(\bullet) +} \sumo k{c\ell r} M^{(\bullet,k)}_t y^{(\bullet,k)}(t)\\
%\coltwo{g^{(j)}_{LS}}{h^{(j)}_{LS}}
%&= Q^{(j)+} \sumo k{c\ell r} [M^{(j,k)}_{\cos,t} y^{(j,k)}_{\cos}(t)
%+ M^{(j,k)}_{\sin,t} y^{(j,k)}_{\sin}(t)].
%\end{align}
%The actual $g^*,h^*$ satisfy
%\begin{align}
%\coltwo{g^*}{h^*}
%&= Q^{(\bullet) +} \sumo k{c\ell r} M^{(\bullet,k)}_t \ol y^{(\bullet,k)}(t)\\
%P^{(j)}\coltwo{g^*}{h^*}
%&= Q^{(j)+} \sumo k{c\ell r} [M^{(j,k)}_{\cos,t} \ol y^{(j,k)}_{\cos}(t)
%+ M^{(j,k)}_{\sin,t} \ol y^{(j,k)}_{\sin}(t)].
%\end{align}
%Subtracting gives
%\begin{align}
%\coltwo{g^{(\bullet)}_{LS}}{h^{(\bullet)}_{LS}}-
%\coltwo{g^*}{h^*}
%&= Q^{(\bullet) +} \sumo k{c\ell r} M^{(\bullet,k)}_t \ol y^{(\bullet,k)}(t)\\
%P^{(j)}\ba{\coltwo{g^{(j)}_{LS}}{h^{(j)}_{LS}} - \coltwo{g^*}{h^*}}
%&= Q^{(j)+} \sumo k{c\ell r} [M^{(j,k)}_{\cos,t} \ol y^{(j,k)}_{\cos}(t)
%+ M^{(j,k)}_{\sin,t} \ol y^{(j,k)}_{\sin}(t)].
%\label{e:err}
%\end{align}
%In section~\ref{s:mat-conc} we lower bound %$Q^{(\bullet)+}$ and
%$Q^{(j)+}$, and in Section~\ref{s:vec-conc} we lower bound % and
%$M^{(j,k)}_{\cos,t} \ol y^{(j,k)}_{\cos}(t)
%+ M^{(j,k)}_{\sin,t} \ol y^{(j,k)}_{\sin}(t)$.


%%%%moved to appendix
%\input{conc}

\subsection{Generalization}
%Rewrite~\eqref{e:err} as
%%Let $Q^{(j)} = \sumo k\ell \sumo t{T}M_t^{(j,k)}M^{(j,k)\top}$. Note 
%\begin{align}
%%\coltwo{g_{LS}}{h_{LS}} - \coltwo{g}{h} &= 
%%Q^{(j)-1}\sumo k\ell \sumo tT M^{(j,k)}\eta^{(j,k)}_{t+1}\\
%P^{(j)}\ba{
%\coltwo{g_{LS}^{(j)}}{h_{LS}^{(j)}} - \coltwo{g}{h}
%}
%&=\Ga^{+\rc 2}(\Ga^{+\rc 2}Q^{(j)} \Ga^{+\rc 2})^{+})\sumo k\ell \sumo tT \ba{\Ga^{+\rc 2} 
%M^{(j,k)}_{\cos,t}\eta^{(j,k)}_{\cos}(t)
%+
%\Ga^{+\rc 2} 
%M^{(j,k)}_{\sin,t}\eta^{(j,k)}_{\sin}(t)
%}
%\end{align}
%By Lemmas~\ref{l:mat-conc} and~\ref{l:vec-conc}, for $\ell \ge C_2^2\pa{r+\ln \prc{\de}}$, 
%\begin{align}
%\Pj\pa{
%\fc 32 \ell T P^{(j)} \succeq {\Ga^{+\rc 2} Q^{(j)} \Ga^{+\rc 2}} \succeq \rc 2 \ell T P^{(j)}
%} &\ge 1-\de\\
%\Pj\pa{
%\sumo k\ell \sumo tT \Ga^{+\rc 2} 
%M^{(j,k)}_{\cos,t}\eta^{(j,k)}(t) \le C_4 \pa{\sqrt r + \sqrt{\ln \pf{4T\ell}{\de}}}\sqrt{\ell T \ln \pf{2}{\de}}
%} &\ge 1-\de\\
%\implies 
%\Pj\pa{\ve{\Ga^{\rc 2} \pa{\coltwo{g_{LS}}{h_{LS}} - \coltwo{g^*}{h^*}}}
%\le \fc{2C_4(\sqrt r + \sqrt{\ln \pf{4T\ell}{\de}})\sqrt{\ln \pf{2}{\de}}}{\sqrt{\ell T}}
%}
%&\ge 1-2\de.
%\end{align}

We now compute the performance of $g^*,h^*$ on the minimax problem.
Let 
\begin{align}
L^{(\bullet)}(h) &= \rc{r}\sumo k{c\ell r} 
\ve{M^{(\bullet, k)\top}(h-h_{LS})}^2
\\
L^{(j)}(g,h) &= \sumo k{\ell}
\ba{ \ve{M^{(j,k)\top}_{\cos}\coltwo gh - y^{(j,k)}_{\cos}}^2
+ \ve{M^{(j,k)\top}_{\sin}\coltwo gh - y^{(j,k)}_{\sin}}^2}
.
\end{align}
Note that
\begin{align}
L^{(\bullet)}(h) - L^{(\bullet)}(h_{LS})
&=(h-h_{LS})^\top Q^{(\bullet)} (h-h_{LS})\\
L^{(j)}(g,h) - L^{(j)}(g_{LS},h_{LS}) &= \pa{\coltwo{g}{h} - \coltwo{g^{(j)}_{LS}}{h_{LS}}}^\top Q^{(j)} \pa{\coltwo{g}{h} - \coltwo{g^{(j)}_{LS}}{h_{LS}}}.
\end{align}
We have that with probability $\ge 1-\de$, by Lemma~\ref{l:mat-conc} and~\eqref{e:gagh0},
\begin{align}
L^{(\bullet)}(h^*) - L^{(j)}(h_{LS}) 
&\le \rc r\ve{\Ga^{(\bullet)-\rc 2} Q^{(\bullet)} \Ga^{(\bullet)-\rc 2}} \ve{\Ga^{(\bullet)\rc 2} (h^*-h_{LS})}^2\\
&\le 
C_8 \rc{r} (c\ell rT) \rc{c\ell T} \pa{\ln \pf{\ell rT}{\de}}^3
=
C_8 \pa{\ln \pf{\ell rT}{\de}}^3\\
L^{(j)}(g^*,h^*) - L^{(j)}(g^{(j)}_{LS},h_{LS}) 
&\le \ve{\Ga^{(j)+\rc 2} Q^{(j)} \Ga^{(j)+\rc 2}} \ve{\Ga^{(j)\rc 2} \pa{\coltwo{g^*}{h^*} - \coltwo{g_{LS}^{(j)}}{h_{LS}}}}^2\\
&\le 
C_8 \ell T \rc{\ell T} \pa{\ln \pf{\ell rT}{\de}}^3=
C_8\pa{\ln \pf{\ell rT}{\de}}^3.
%6C_4^2\pa{\sqrt r + \sqrt{\ln \pf{T\ell}{\de}}}^2
%{\ln \pf{2}{\de}}.
\end{align}
Because $\coltwo gh$ is the argmin of~\eqref{e:ls}, we have 
$L^{(\bullet)}(h) -L^{(\bullet)}(h^*)\le C_8\pa{\ln \pf{\ell rT}{\de}}^3$, and similarly for $L^{(j)}$. Hence
\begin{align}
\ve{\Ga^{(\bullet)\rc 2}(h-h^*)}^2
%& \le \fc{2C_8}{\ell T}\ve{Q^{(\bullet)\rc 2}(h-h^*)}_2^2\\
%&\le \fc{4C_8}{\ell T} \pa{\ve{Q^{(\bullet)\rc 2}(h-h_{LS})}^2 + \ve{Q^{(\bullet)\rc2}(h_{LS}-h^*)}}\\
&\le 2\pa{\ve{\Ga^{(\bullet)\rc 2}(h-h_{LS})}^2 + \ve{\Ga^{(\bullet)\rc2}(h_{LS}-h^*)}}\\
&\le 2\pa{\ve{Q^{(\bullet)-\rc 2}\Ga^{(\bullet)} Q^{(\bullet)-\rc 2}}
\ve{Q^{(\bullet)\rc2}(h-h_{LS})}_2^2
+ \ve{\Ga^{(\bullet)\rc2}(h_{LS}-h^*)}
}\\
&\le \fc{C_9}{c\ell T}\pa{\ln \pf{\ell rT}{\de}}^3
%&\le \fc{C_9}{\ell T}\pa{\ln \pf{\ell rT}{\de}}^3
\end{align}
%
%
%$L^{(j)}(g,h) - L^{(j)}(g^{(j)}_{LS}, h^{(j)}_{LS})
%\le 
%L^{(j)}(g^*,h^*) - L^{(j)}(g^{(j)}_{LS},h^{(j)}_{LS}) 
%$
%Then 
and similarly
\begin{align}
\ve{\Ga^{(j)\rc 2}\pa{\coltwo gh - \coltwo{g^*}{h^*}}}_2^2
%&\le \fc{2}{\ell T}\ve{Q^{(j)\rc 2}\pa{\coltwo gh - \coltwo{g^*}{h^*}}}_2^2\\
%&\le \fc{4}{\ell T}\pa{
%\ve{Q^{(j)\rc 2}\pa{\coltwo gh - \coltwo{g^{(j)}_{LS}}{h_{LS}}}}^2
%+
%\ve{Q^{(j)\rc 2}\pa{\coltwo{g^{(j)}_{LS}}{h_{LS}}-\coltwo{g^*}{h^*}}}^2
%}\\
&\le 
%\ub{4\cdot 6C_4^2}{C_5}\rc{\ell T}\pa{\sqrt r + \sqrt{\ln \pf{T\ell}{\de}}}^2
%{\ln \pf{2}{\de}}
\fc{C_9}{\ell T} \pa{\ln \pf{\ell rT}{\de}}^3.
\end{align}
%\fixme{Talk about noise}
Now $\ve{\Ga^{(\bullet)\rc 2}(h-h^*)}_2^2$ represents the mean square estimation error when the input is 0, so 
\begin{align}
\ve{(H-H^*)H^*_{\textrm{unr}}}_2&=
\ve{\Ga^{(\bullet)\rc 2}(h-h^*)}\le
 \fc{C_{10}}{\sqrt{\ell T}}\pa{\ln \pf{c\ell rT}{\de}}^{\fc32}
\end{align}

We can decompose 
\begin{align}
M^{(j,k)}_{\cos,t} &=\ub{\coltwo{x^{(j,k)}_{\cos}(t-1:t-r)}{y_{(x^{(j,k)}_{\cos},0)}(t-1:t-r)}}{\E M^{(j,k)}_{\cos,t}} + \coltwo{0}{y_{(0,\eta^{(j,k)}_{\cos})}(t-1:t-r)}
\end{align}
and similarly for $\sin$.
Consider the response to $x(t) = e^{\fc{2\pi ijt}{cr}}$, $j\le \fc{cr}2$, with noise $\eta^{(j)}(t)=\eta^{(j)}_{\cos}(t)+i\eta^{(j)}_{\sin}(t)$. %(Although we cannot put in complex values in the system, there is a well-defined response for complex inputs.) Suppose the noise is $\eta$. 
Let $M^{(j,k)}_t = \coltwo{x(t-1:t-r)}{y(t-1:t-r)}$. We can similarly decompose $M^{(j,k)}_t$; the mean response is $\E M^{(j,k)}_t = \E [M^{(j,k)}_{\cos,t}+ iM^{(j,k)}_{\sin,t}]$. We obtain an upper bound on the difference in the mean responses:
\begin{align}
&
\pa{\coltwo gh - \coltwo{g^*}{h^*}}^\top 
%\rc T\sumo tT 
(\E M^{(j,k)}_t)(\E M^{(j,k)}_t)^\top 
\pa{\coltwo gh - \coltwo{g^*}{h^*}}\\
&=
\pa{\coltwo gh - \coltwo{g^*}{h^*}}^\top 
%\rc T\sumo tT 
\E [M^{(j,k)}_{\cos,t}- iM^{(j,k)}_{\sin,t}]\E[M^{(j,k)}_{\cos,t}+ iM^{(j,k)}_{\sin,t}]^{\top} 
\pa{\coltwo gh - \coltwo{g^*}{h^*}}\\
&\le %\rc{\ell T}
\ve{\Ga^{(j)\rc 2}\pa{\coltwo gh - \coltwo{g^*}{h^*}}}_2^2\\
&\le 
%\fc{C_5}{\ell T}
%\pa{\sqrt r + \sqrt{\ln \pf{T\ell}{\de}}}^2{\ln \pf{2}{\de}}.
\fc{C_9}{\ell T} \pa{\ln \pf{\ell rT}{\de}}^3.
\end{align}
Since the mean square response is exactly $\ab{[(G-G^*) + (H-H^*) H^*_{\textrm{unr}}G^*](e^{\fc{2\pi ij}{cr}})}^2$, we get 
\begin{align}\label{e:bd-all-freqs}
\ab{[(G-G^*) + (H-H^*) H^*_{\textrm{unr}}G](e^{\fc{2\pi ij}{cr}})}
&\le  %\sfc{C_5}{\ell T}\pa{\sqrt r + \sqrt{\ln \pf{T\ell}{\de}}}\sqrt{\ln \pf{2}{\de}}.
\fc{C_{10}}{\sqrt{\ell T}} \pa{\ln \pf{\ell rT}{\de}}^{\fc32}.
\end{align}
Note the same inequality holds for $j$ replaced by $r-j$ and $M^{(j,k)}_{\cos,t}+ iM^{(j,k)}_{\sin,t}$ replaced by $M^{(j,k)}_{\cos,t}- iM^{(j,k)}_{\sin,t}$, so~\eqref{e:bd-all-freqs} holds for all $j\in \Z$.

\subsection{Interpolation}

\begin{lem}\label{l:interp}
Let $Q(z):= \sumz k{r-1} a_k z^{k}$, where $a_k\in \C$. 
\begin{enumerate}
\item
\cite[Theorem 15.2]{trefethen2013approximation}
For any $N\ge r$, $\ve{Q}_\iy\le \pa{\fc{2}{\pi}\ln (r+1)+1} \max_{j=0,\ldots, N-1} |Q(e^{\fc{2\pi i j}{N}})|$.
\item
\citep{bhaskar2013atomic}
For any $N\ge 4\pi r$, $\ve{Q}_\iy \le \pa{1+\fc{4\pi r}{N}} \max_{j=0,\ldots, N-1} |Q(e^{\fc{2\pi i j}{N}})|$. 
\end{enumerate}
\end{lem}
From~\eqref{e:bd-all-freqs} we get that for $\ep=\fc{C_{10}}{\sqrt{\ell T}}\pa{\ln \pf{\ell r T}{\de}}^{\fc32}$, $\om=e^{\fc{2\pi i}{cr}}$, $j\in \Z$, that
\begin{align}
\ab{[(G-G^*) + (H-H^*) G^* H^*_{\textrm{unr}}](\om^j)} &\le \ep\\
\implies
\ab{[(G-G^*)(1-z^{-1}H^*) + (H-H^*)G^*](\om^j)} &\le \ep \ab{1-\om^{-j}H^*(\om^j)} \le \ep(1+\ve{H^*}_\iy).
\end{align}
Suppose $c>8\pi$. 
By Lemma~\ref{l:interp}, since $(G-G^*)(1-z^{-1}H^*) + (H-H^*)G^*$ has degree $\le 2r$ in $z^{-1}$, 
\begin{align}
\ve{(G-G^*)(1-z^{-1}H) + (H-H^*)G^*}_\iy &\le \ep\pa{1+\fc{8\pi}{c}} (1+\ve{H^*}_\iy)\\
\implies
\ve{(G-G^*) + (H-H^*)G^*H^*_{\textrm{unr}}}_\iy &\le \ep\pa{1+\fc{8\pi}{c}} (1+\ve{H^*}_\iy)\ve{H^*_{\textrm{unr}}}_{\iy}.
\end{align}

This finishes the proof of Theorem~\ref{t:main}.
%%%%%%%%%%%%%%%
\begin{comment}

\subsection{Truncation error}

\begin{proof}[Proof of Theorem~\ref{t:main-trunc}]
If $D_1,D_2$ are two distributions on $\Om$ with TV-distance $\le \de$, and $\cal A$ is any algorithm with input space $\Om$, then $\cal A(x), x\sim D_1$ and $\cal A(x), x\sim D_2$ also have TV-distance $\le \de$.

Consider Algorithm~\ref{a:ls} run with signals $x_{\iy}$ stretching back to $-\iy$ and signals $x_{\ge -L}$ only stretching back to $-L$. Consider the distributions they induce on the $y(t)$. As long as we choose $L$ so that the TV-distance between those distributions is $\le \fc{\de}2$, then we can apply Theorem~\ref{t:main} with $\fc{\de}2$ to get the desired result.

Let $y_\iy$ and $y_{\textrm{fin}}$ be the output signals given input signals $x_{\iy}$ and $x_{\ge -L}$, and noise $\eta_{\iy}$ and $\eta_{\ge-L}$. We have
\begin{align}
y_\iy(t+1) &= g^**x_\iy(t) + h_{\textrm{unr}}^**h^**\eta_{\cos}(t)\\
y_{\textrm{fin}}(t+1) &=g^**(x_\iy \one_{\ge -L}) (t) + (h_{\textrm{unr}}^**h^**(\eta_\iy\one_{\ge -L})(t)\\
&=[g_{L+t}^**x_\iy](t) + [(h_{\textrm{unr}}^**h^*)_{L+t}*\eta_\iy](t)\\
%\ze(t):= 
y_\iy(t+1)-y_{\textrm{fin}}(t+1)&=
[g^*_{>L+t} * x_\iy] (t)
+ [(h_{\textrm{unr}}^**h^*)_{>L+t}*\eta_\iy](t)
\end{align}
The first term has magnitude at most $\ve{g^*_{>L+t}}_1\ve{x_\iy}_\iy\le \fc{\de}{8c\ell rT}$ and the second term is normally distributed with variance $\le \ve{(h_{\textrm{unr}}^* * h^*)}_2^2\le \ve{(h_{\textrm{unr}}^* * h^*)}_1^2\le \fc{\de}{8c\ell rT}$, by the condition on $L$ and Lemma~\ref{l:suff-l}. Thus the distributions of $y_\iy(t+1)$ and $y_{\textrm{fin}}(t+1)$ are gaussians whose mean differ by $\le \de' = \fc{\de}{8c\ell rT}$. The variance of $y_\iy(t+1)$ is 1 and the variance of $y_{\textrm{fin}}(t+1)$ is in $[1,{\de'}2]$.

By the following bound on KL-divergence,
\begin{align}
\KL(N(\mu_1,\si_1^2)||N(\mu_2,\si_2^2)) 
&\le \ln \pf{\si_2}{\si_1} + \fc{\si_1^2+(\mu_1-\mu_2)^2}{2\si_2^2}-\rc 2,
\end{align}
and Pinsker's inequality, letting $\cal D(\cdot)$ denote the distribution of a random variable, 
\begin{align}
\KL(\cal D(y_\iy(t+1))|\cal D(y_{\textrm{fin}}(t+1)))
&\le \ln \prc{\sqrt{1+\de^{\prime2}}}
+\fc{1+\de^{\prime2}+\de^{\prime2}}2-\rc 2\le 2\de' = \fc{\de}{4c\ell rT}.
\end{align}
Thus the TV-distance between the $y(1:T)$ of all the rollouts is at most $\fc{\de}2$, as needed.
\end{proof}
\end{comment}

%%%%%%%%%%%

==> proof_old.tex <==
\section{Proof}
\label{s:proof}

We prove Theorem~\ref{t:main}. We consider the case where $r$ is odd. The case where $r$ is even can be obtained from simple modifications of the proof.
First, we compute the argmin of~\eqref{e:ls}-\eqref{e:ls2}.
\begin{align}\label{e:amin}
\coltwo{\wh g}{\wh h} 
&= 
\ub{\pa{
\sumo jr N^{(j)\top} N^{(j)} + M^{(0)\top}M^{(0)} + \sumo j{r/2}\pa{M^{(j)\top}_{\cos} M^{(j)}_{\cos} + M^{(j)\top}_{\sin} M^{(j)}_{\sin}
}}}{=:Q}^{-1}\\
&\quad 
\pa{
\sumo jr N^{(j)\top} w^{(j)}(r:T) + M^{(0)\top}y^{(0)}(r:T) + \sumo j{r/2}\pa{M^{(j)\top}_{\cos} y^{(j)}_{\cos}(r:T) + M^{(j)\top}_{\sin} y^{(j)}_{\sin}}}.
\label{e:amin2}
\end{align}
Let $\ol w^{(j)}$ be the predicted output for the rollout with input $z^{(j)}$: $\ol w^{(j)} = \cancel{g^**z^{(j)}(t)} + h^**w^{(j)}(t)$, and similarly define $\ol y^{(0)}$, $y^{(j)}_{\cos}$, and $y^{(j)}_{\sin}$. 
Let $\xi^{(j)}$, $\eta^{(0)}$, $\eta^{(j)}_{\cos}$, and $\eta^{(j)}_{\sin}$ be the noise in each of the rollouts, so that $\xi^{(j)} = w^{(j)} - \ol w^{(j)}$ and so forth. 
Then from~\eqref{e:amin}-\eqref{e:amin2},
\begin{align}\label{e:err}
\coltwo{\wh g}{\wh h} - \coltwo{\wh g^*}{\wh h^*} 
&= \pa{
\sumo jr N^{(j)\top} N^{(j)} + M^{(0)\top}M^{(0)} + \sumo j{r/2}\pa{M^{(j)\top}_{\cos} M^{(j)}_{\cos} + M^{(j)\top}_{\sin} M^{(j)}_{\sin}
}}^{-1}
\\
&\quad 
\pa{
\sumo jr N^{(j)\top} \xi^{(j)}(r:T) + M^{(0)\top}\eta^{(0)}(r:T) + \sumo j{r/2}\pa{M^{(j)\top}_{\cos}  \eta^{(j)}_{\cos}(r:T) + M^{(j)\top}_{\sin} \eta^{(j)}_{\sin}}}.
\label{e:err2}
\end{align}

\subsection{Changing basis}

We consider the system response $y_{x,0}$ for $x(t) = e^{\fc{2\pi i jt}{r}}$, $t\in \Z$ and zero noise. (Although we cannot put in complex values in the system, there is a well-defined response for complex inputs.) Then because convolution is multiplication in the Fourier domain, $y(t+1) = \wh h^*\wh g^*(j) e^{\fc{2\pi i jt}{r}}$. We show by a change of basis that we can reduce to the case where $a_j:=\wh h^* \wh g^*(j)=0$. 

Let $S = \matt{I_r}{-\diag(a_0,\ldots, a_{r-1})}{O_r}{I_r}$. We break each of the outputs into the response from the input and the response from the noise, for example,
\begin{align}
y^{(j)}_{\sin} &= y_{x^{(j)}_{\sin}, \eta^{(j)}_{\sin}} = y_{x^{(j)}_{\sin},0} + y_{0,\eta^{(j)}_{\sin}}\\
u^{(j)}_{\sin} &= u_{x^{(j)}_{\sin}, \eta^{(j)}_{\sin}} = u_{x^{(j)}_{\sin},0} + u_{0,\eta^{(j)}_{\sin}}
\end{align}
Doing this decomposition gives
\begin{align}
N^{(j)}_t &= e_2 \ot \wh v^{(j)}_t\\
M^{(0)}_t &= e_1\ot e_0 +a_0(e_2\ot e_0) + e_2 \ot \wh u_{0,\eta^{(j)}_{\cos},t}\\
M^{(j)}_{\cos,t} &= e_1\ot \pf{e_j+e_{r-j}}2 + e_2\ot \pf{a_je_j+\ol a_j e_{r-j}}2 + e_2 \ot \wh u_{0,\eta^{(j)}_{\cos},t}\\
M^{(j)}_{\sin,t} &= e_1\ot \pf{e_j-e_{r-j}}{2i} + e_2\ot \pf{a_je_j-\ol a_j e_{r-j}}{2i} + e_2 \ot \wh u_{0,\eta^{(j)}_{\cos},t}
\end{align}
Changing basis gives
\begin{align}
N^{(j)}_tS &= N^{(j)}_t = e_2 \ot \wh v^{(j)}_t\\
M^{(0)}_tS &=e_1\ot e_0 + e_2 \ot \wh u_{0,\eta^{(0)},t}\\
M^{(j)}_{\cos,t}S &= e_1\ot \pf{e_j+e_{r-j}}2 + e_2 \ot \wh u_{0,\eta^{(j)}_{\cos},t}\\
M^{(j)}_{\sin,t}S &= e_1\ot \pf{e_j-e_{r-j}}{2i}  + e_2 \ot \wh u_{0,\eta^{(j)}_{\cos},t}
\end{align}
Then we can write $Q$ as $Q=S[S^\dagger QS]^{-1} S^\dagger$.
Using $aa^\dagger + bb^\dagger = \rc 2(a-b)(a-b)^\dagger + \rc 2 (a+b)(a+b)^\dagger$  we further rewrite
\begin{align}
S^\dagger M^{(j)\dagger}_{\cos} M^{(j)}_{\cos} S
+ 
S^\dagger M^{(j)\dagger}_{\sin} M^{(j)}_{\sin} S
&=
\rc 2 [M^{(j)\dagger} M^{(j)} + M^{(r-j)\dagger}M^{(r-j)}]\\
\text{where }
M^{(j)} &= e_1\ot e_j + e_2 \ot (\wh u_{0, \eta^{(j)}_{\cos},t} + i \wh u_{0, \eta^{(j)}_{\sin}, t})\\
M^{(r-j)} &= e_1\ot e_{r-j} + e_2 \ot (\wh u_{0, \eta^{(j)}_{\cos},t} - i \wh u_{0, \eta^{(j)}_{\sin}, t})\\
\end{align}

\subsection{Applying the Small-Ball inequality}

\begin{lem}\label{l:trans-bd}
Let $T=\matt{(0^{r-1})^\top}0{I_{r-1}}{0^{r-1}}$. Then $\sumz j{r-1} (T^jv)(T^jv)^\top \succeq \rc{2\ve{v}_1^2+1}I_r$. 
\end{lem}
\begin{proof}
To be added. It suffices to show that every square submatrix in the upper left corner of $\sumz j{r-1} (T^jv)(T^jv)^\top - \rc{2\ve{v}_1^2+1}I_r$ has nonnegative determinant. Apply elementary row and column operations so that the only terms off the diagonal are $\ep$ terms. Use Gerschgorin's Disk Theorem.
\end{proof}

\begin{lem}
Let $\cal F_j$ have the information for the $\eta(k)$, $k\le j$ for all the sequences. Suppose that $\ve{\hunr}_1\le L$. Fix $w$. Then
\begin{align}
\E\ba{
\sumo jT |w^\dagger S^\dagger N^{(j)\dagger}_{s+r}|^2 +
|w^\dagger S^\dagger M^{(0)\dagger}_{s+r}|^2+
\rc 2 \sumo j{r/2} \pa{|w^\dagger S^\dagger M^{(j)\dagger}_{s+r}|^2+
|w^\dagger S^\dagger M^{(r-j)\dagger}_{s+r}|^2
}|\cal F_r
}
&\succeq 
\fc{r}3 \matt{I_d}{}{}{\rc{2L^2+1}I_d}.
\end{align}
\end{lem}
\begin{proof}
We can replace $w^\dagger$ by $w^\dagger \matt{I}{}{}{F^\dagger}$ and $S^\dagger$ by $\matt{I}{}{}F S^\dagger$ where $F$ is the Fourier change-of-basis matrix. Now
\begin{align}
N^{(j)}_tS\matt{I}{}{}F &= N^{(j)}_t = e_2 \ot v^{(j)}_t\\
M^{(0)}_tS\matt{I}{}{}F &=e_1\ot e_0 + e_2 \ot  u_{0,\eta^{(0)},t}\\
M^{(j)}_{t}S\matt{I}{}{}F &= e_1\ot {e_j} + e_2 \ot (u_{0,\eta^{(j)}_{\cos},t}+iu_{0,\eta^{(j)}_{\sin},t})\\
M^{(r-j)}_{t}S\matt{I}{}{}F &= e_1\ot {e_{r-j}} + e_2 \ot (u_{0,\eta^{(j)}_{\cos},t}-iu_{0,\eta^{(j)}_{\sin},t})
\end{align}

We use the following fact: if $\E v_iv_i^\dagger = \E w_iw_i^\dagger$, then $\E \sumo iT (u+v_i)(u+v_i)^\dagger + w_iw_i^\dagger \succeq \rc 3 T uu^\top + \rc 3 \sumo iT \E v_iv_i^\dagger$. This follows from
\begin{align}
\E \sum_i uu^\dagger + (u^\dagger v_i+v_i^\dagger u) + 2v_iv_i^\dagger &\succeq \E \sum_i \rc 3 (uu^\dagger + v_iv_i^\dagger)\\
\Leftarrow
\E \sum_i \fc 23 uu^\dagger + (u^\dagger v_i+v_i^\dagger u) + \fc 53v_iv_i^\dagger &\succeq 0.
\end{align}
Applying this gives  \fixme{fix indexing}
\begin{align}
\matt I{}{}F S^\dagger N^{(j)\dagger}_t N^{(j)}_t S \matt I{}{}{F^{\dagger}}
+
\matt I{}{}F S^\dagger N^{(j)\dagger}_t M^{(j)}_t S \matt I{}{}{F^{\dagger}}
&\succeq 
\fc r3 (e_1\ot e_j)^\top (e_1\ot e_j) + \rc 3 \E (e_2\ot v^{(j)}_t)^\dagger(e_2\ot v^{(j)}_t).
\end{align}
By Lemma~\ref{l:trans-bd},
\begin{align}
\E(v^{(j)\dagger}_{s+r} v^{(j)}_{s+r}|\cal F_s)
&\succeq \Var(v^{(j)\dagger}_{s+r} v^{(j)}_{s+r} |\cal F_s)\\
&\succeq \rc{2L^2+1}I_d
\end{align}
Putting this together gives
\begin{align}
\E\ba{
\sumo jT |w^\dagger S^\dagger N^{(j)\dagger}_{s+r}|^2 +
|w^\dagger S^\dagger M^{(0)\dagger}_{s+r}|^2+
\rc 2 \sumo j{r/2} \pa{|w^\dagger S^\dagger M^{(j)\dagger}_{s+r}|^2+
|w^\dagger S^\dagger M^{(r-j)\dagger}_{s+r}|^2
}|\cal F_r
}
&\ge\rc3 \sumo j{r} \matt{rE_jj}{}{}{\rc{2L^2+1}I_d} = \fc r3 \matt{I_d}{}{}{\rc{2L^2+1}I_d}.
\end{align}
\end{proof}

\begin{cor}
The sequences $u^{(j)}_t$ \fixme{(taken together)} satisfy the $(2r, \fc{r}{3(2L^2+1)}I_r,\fc{3}{20})$-BMSB condition. 
\end{cor}
\begin{proof}
The $(k,\nu I_r, p)$-BMSB condition says that for any $w\in \bS^{r-1}$, 
\begin{align}
\rc k \sumo tk \sumz j{r-1} \Pj\pa{|\an{w,u^{(j)}_{s+t}}|\ge \nu | \cal F_s}&\le p
\end{align}
where $\cal F_s = \si(u^{(j)}_0,\ldots, u^{(j)}_s, 0\le j<r)$. 
%For $t\ge r$, $u_{s+t}$ is independent of $\cal F_s$, and is distributed as $N(0,I_r)$. Hence
\fixme{??? hence}
\begin{align}
\rc{2r} \sum_{t=1}^{2r}\sumz j{r-1}  \Pj\pa{|\an{w,u^{(j)}_{s+t}}|\ge \fc{r}{3(2L^2+1)} | \cal F_s}&\ge
\rc{2r} \sum_{t=r}^{2r}\sumz j{r-1}  \Pj\pa{|\an{w,u^{(j)}_{s+t}}|\ge \fc{r}{3(2L^2+1)}  |\cal F_s}\\
& = \rc{2r} \sum_{t=r}^{2r} \Pj_{X\sim N(0,1)} (|X|\ge 1)\\
& \ge \rc 2\cdot \fc{3}{10} = \fc{3}{20}
\end{align}
by the Paley-Zygmund inequality.
\end{proof}

Then by Lemma~\ref{l:bmsb-mat}, 
\begin{align}
\Pj\pa{Q\succeq \fc{rp^2}{48(2L^2+1)}I_r} &\ge 1-\de - \exp\pa{d\ln \pf{72 d\cdot 3(2L^2+1)}{rp^2\de} - \ff{T}{k}p^2/8}.
\end{align}
\subsection{Bounding the error}
We've bounded $Q^{-1}$ from above; now we bound~\eqref{e:err2}.
Note
\begin{align}
\ve{N^{(j)}_tS} &=\ve{\wh v^{(j)}_t}\\
\ve{M^{(0)}_tS} &= \sqrt{1+ \ve{\wh u_{0,\eta^{(0)},t}}^2}\\
\ve{M^{(0)}_{\cos,t}S} &= \sqrt{\rc2 + \ve{\wh u_{0,\eta^{(0)}_{\cos},t}}^2}\\
\ve{M^{(0)}_{\sin,t}S} &= \sqrt{\rc2 + \ve{\wh u_{0,\eta^{(0)}_{\sin},t}}^2}.
\end{align}
Now $y_{(0,\eta)} (t) = \hunr * \eta(t)$ and 
\begin{align}
\E[(\hunr * \eta(t+s))^2] = \sumz k{\iy} \hunr (k)^2 \le L^2
\end{align}
so 
\begin{align}
\Pj\pa{\exists t, \max\bc{ |w^{(j)}(t)|, |y^{(0)}(t)|,  |y^{(j)}_{\cos}(t)|, |y^{(j)}_{\sin}(t)|}>\sqrt{2\ln \pf{8Tr}{\de}}L}
&\le 2Tr \exp\pa{-\fc{2\ln \pf{8Tr}{\de}L^2}{2L^2}}&=\fc{\de}4.
\end{align}
Then by Azuma's inequality, ...\fixme{fix this application}

\subsection{Interpolation}

We use the following theorem from numerical analysis.
\begin{thm}[Lebesgue constant of equispaced points on unit circle]
Let $p$ be a polynomial of degree $r$ passing through $(e^{\fc{2\pi i j}{r}}, z_r)$ for $0\le j<r$. Then 
\begin{align}
\fc{\max_{\ve{z}=1}|p(z)|}{\max_r |z_r|}\le \fc{2}{\pi}\ln (r+1)+1.
\end{align}•
\end{thm}
